Neural Retriever and Go Beyond: A Thesis Proposal

Information Retriever (IR) aims to find the relevant documents (e.g. snippets, passages, and articles) to a given query at large scale. IR plays an important role in many tasks such as open domain question answering and dialogue systems, where external knowledge is needed. In the past, searching algorithms based on term matching have been widely used. Recently, neural-based algorithms (termed as neural retrievers) have gained more attention which can mitigate the limitations of traditional methods. Regardless of the success achieved by neural retrievers, they still face many challenges, e.g. suffering from a small amount of training data and failing to answer simple entity-centric questions. Furthermore, most of the existing neural retrievers are developed for pure-text query. This prevents them from handling multi-modality queries (i.e. the query is composed of textual description and images). This proposal has two goals. First, we introduce methods to address the abovementioned issues of neural retrievers from three angles, new model architectures, IR-oriented pretraining tasks, and generating large scale training data. Second, we identify the future research direction and propose potential corresponding solution.

==> publication.tex <==
\begin{table*}[t]
    \centering 
    \small
\resizebox{0.94\linewidth}{!}{
    \begin{tabular}{@{}p{0.35\linewidth}p{0.15\linewidth}p{0.1\linewidth}p{0.4\linewidth}@{}}
        \toprule
        \textbf{Short Title} & \textbf{Venue} & \textbf{Domain} & \textbf{Keywords} \\
        \toprule
        LPMLN 
        & ICLP-2019
        & LP
        & Knowledge Representation and Reasoning. \\
    \midrule
    VQA Semantic Evaluation
        & EACL-2021
        & V+L
        & VQA, Semantic Evaluation. \\
    \midrule
    Retriever-Reader for OKVQA
        & EMNLP-2021
        & V+L
        & Knowledge-based VQA, visual retriever, visual reader, weak-supervised learning. \\
    \midrule
    Neural Retriever in Biomedical Domain & AAAI-2022 & L & retrieval, question generation, pretraining-task, poly-dpr, biomedical. \\
    \midrule
    Transformers for Action Reasoning & arXiv-2020 & L & Reasoning about action, generalization, transformers. \\
    \midrule
    Joint Model for QA Task & arXiv-2021 & L & QA, multi-task learning, joint model. \\
    \midrule
    SCONER & ARR-2021 (under reivew) & L & Retrieval-based QA, neural-reranker, multi-domain learning, data augmentation, label generation, generalization.\\
    \midrule
    Generalization and Robustness & ARR-2021 (under reivew) & V, L & Generalization, robustness, NLI, QA, image classification. \\
    \bottomrule
    \end{tabular}
    }
    \caption{Author's publication. LP: logic programming, V: vision, L: language.
    % BM25~\cite{Robertson2009ThePR} and Dense Passage Retrieval~\cite{Karpukhin2020DensePR}.
    }
    \label{tab:publication}
\end{table*}

